A Case Study Analysis for Designing a Lunar Navigation Satellite System with Time-Transfer from Earth-GPS

Recently, there has been a growing interest in the use of a SmallSat platform for the future Lunar Navigation Satellite System (LNSS) to allow for cost-effectiveness and rapid deployment. However, many design choices are yet to be finalized for the SmallSat-based LNSS, including the onboard clock and the orbit type. As compared to the legacy Earth-GPS, designing an LNSS poses unique challenges: (a) restricted Size, Weight, and Power (SWaP) of the onboard clock, which limits the timing stability; (b) limited lunar ground monitoring stations, which engenders a greater preference toward stable LNSS satellite orbits. In this current work, we analyze the trade-off between different design considerations related to the onboard clock and the lunar orbit type for designing an LNSS with time-transfer from Earth-GPS. Our proposed time-transfer architecture combines the intermittently available Earth-GPS signals in a timing filter to alleviate the cost and SWaP requirements of the onboard clocks. Specifically, we conduct multiple case studies with different grades of low-SWaP clocks and various previously studied lunar orbit types. We estimate the lunar User Equivalent Range Error (UERE) metric to characterize the ranging accuracy of signals transmitted from an LNSS satellite. Using the Systems Tool Kit (STK)-based simulation setup from Analytical Graphics, Inc. (AGI), we evaluate the lunar UERE across various case studies of the LNSS design to demonstrate comparable performance as that of the legacy Earth-GPS, even while using a low-SWaP onboard clock. We further perform sensitivity analysis to investigate the variation in the lunar UERE metric across different case studies as the Earth-GPS measurement update rates are varied.

==> old_sections/experiments.tex <==
\section{Our Case Study Analysis: Results and Discussion -- By 11:30PM} \label{sec:experiment_results}
We analyze the trade-off between different design considerations for designing an LNSS with time-transfer from Earth-GPS. 
To do this, we evaluate various case studies related to the onboard clock and the orbit type, which were listed earlier in Section~\ref{sec:simulation_modeling}.

\subsection{Implementation Details} \label{sec:implementation_details}
We design our timing filter with an update period of $\sampinterval=60$~\si{s}, which is equivalent to the rate at which the position and velocity of Earth-GPS and LNSS satellites are sampled from STK software.
%As explained earlier in Section~\ref{sec:simulation_modeling}, an Earth-GPS satellite is considered to be visible if $C/N0>15~$ dB-Hz~(conservative threshold) for at least $40~$s, which indicates the tracking time required by the receiver. 
In the formulation of the measurement noise covariance matrix for our timing filter described earlier in Eqs.~\eqref{eq:measurementnoisecovariance} and for simulating the received pseudorange and pseudorange rate measurement explained previously in Section~\ref{sec:simulation_modeling}, we set the parameters of the DLL and PLL tracking loop errors as follows~\cite{capuano2016gnss}: $\bwcodeloop=0.5$~\si{Hz}, $\corrspace=0.3$~\si{chips}, $\inttime=20$~\si{ms}, $\bwfe=26$~\si{MHz} and $\bwpll=0.5$~\si{Hz}. 
Note that these parameters are set to the same values as that considered in our earlier work~\cite{bhamidipati2021design}.  

To characterize the lunar UERE from Section~\ref{ssec:algorithm_lunarURE}, we consider the same group delay and receiver noise error magnitudes as with the Earth-GPS system, i.e. $\stdlunargd = 0.15$~\si{m} and $\stdlunarrec=0.1$~\si{m}.
Compared to Earth-GPS, which is a terrestrial navigation system with extensive military applications, the LNSS will have greater limitations on ground infrastructure and financial investment to monitor the lunar system.
So, we perform case study analysis by scaling the error component due to the broadcast ephemeris in the lunar UERE as $\stdlunareph=3$~\si{m}, which is essentially one order of magnitude higher in comparison to that of Earth-GPS.  
%So, we also perform sensitivity analysis for each case study by scaling the error component due to the broadcast ephemeris in the lunar UERE as follows:~$\stdlunareph=0.3,~3,~30~$m, where the broadcast ephemeris error component considered for Earth-GPS system is $0.3~$m.  
% So, in addition to analyzing the case studies across , we also perform sensitivity analysis by scaling the error due to the broadcast ephemeris by one order of magnitude in comparison to Earth-GPS, i.e. $\stdlunareph=3$~m.

\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/ELFO_FullSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{ELFO: Full satellite visibility}
		\label{fig:elfo_fullsatvis}
	\end{subfigure}	
	\hspace{2mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/ELFO_SubSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{ELFO: Zoomed-in satellite visibility}
		\label{fig:elfo_subsatvis}
	\end{subfigure}
	\vfill
	\vspace{5mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/NRHO_FullSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{NRHO: Full satellite visibility}
		\label{fig:nrho_fullsatvis}
	\end{subfigure}
	\hspace{1mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/NRHO_SubSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{NRHO: Zoomed-in satellite visibility}
		\label{fig:nrho_subsatvis}
	\end{subfigure}	
	\vfill
	\vspace{5mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/LLO_FullSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{LLO: Full satellite visibility}
		\label{fig:llo_fullsatvis}
	\end{subfigure}
	\hspace{1mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/LLO_SubSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{LLO: Zoomed-in satellite visibility}
		\label{fig:llo_subsatvis}
	\end{subfigure}	
	\vfill
	\vspace{5mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/PCO_FullSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{PCO: Full satellite visibility}
		\label{fig:pco_fullsatvis}
	\end{subfigure}
	\hspace{1mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/PCO_SubSatVis_withAtmMask_withTrackDelay_noLTD.png}
		\caption{PCO: Zoomed-in satellite visibility}
		\label{fig:pco_subsatvis}
	\end{subfigure}	
	\caption{Earth-GPS satellite visibility and maximum ECOP across different orbit types, where blue dotted lines indicate the number of visible Earth-GPS satellites and the red vertical bars indicate regions of ECOP; 
	a), c), e) and g) show the satellite visibility for the entire time duration in ELFO, NRHO, LLO and PCO, respectively; 
	b), d), f) and h) show the zoomed-in satellite visibility for a shorter time segment of $2$ days. 
	We observe that NRHO not only exhibits a least maximum ECOP of $420$~~\si{s} but also the greatest at least one satellite visibility of $99.9\%$.}
	\label{fig:experiment_maximum_timing_errors}
\end{figure}

\subsection{Validation Metrics} 
To perform comparison analysis across different case studies, we define the following four validation metrics: 
\begin{enumerate}
    \item Satellite visibility, which indicates the percentage time in the entire experiment duration for which the number of visible Earth-GPS satellites are greater than a pre-specified threshold;
    \item Maximum ECOP to identify the region of maximum continuous time when no Earth-GPS satellites are visible; 
    \item Root-Mean-Square~(RMS) errors in clock estimates to analyze the performance of our time-transfer from Earth-GPS; and
    \item Value of lunar UERE metric to characterize the ranging measurement accuracy of signals transmitted by an LNSS satellite. Recollect from an earlier explanation in Section~\ref{sec:proposed_time_transfer_technique} that the lunar UERE metric depends on the RMS error in clock bias. 
\end{enumerate}

To characterize the satellite visibility for a given lunar orbit, we examine the percent time in which a certain minimum number of Earth-GPS satellites are visible. 
In particular, we examine the percent of time that at least $1$ Earth-GPS satellite is visible, since this is the minimum number required to correct the clock estimates, as well as the percent time that at least $4$ Earth-GPS satellites are visible, since this is the minimum number to perform full state estimation involving position, clock bias, velocity and clock drift. 
We consider a particular case study, i.e., an orbit-clock pair for an LNSS satellite, to be desirable if it exhibits either some or all of the following: greatest satellite visibility, least maximum ECOP, and least lunar UERE. 

\subsection{Across Orbit Types: Variation in Satellite Visibility and Maximum ECOP}
For the four orbit types considered in our case study, we showcase the number of visible Earth-GPS satellites by blue in Figs.~\ref{fig:elfo_fullsatvis}-\ref{fig:pco_subsatvis} while the highlighted red vertical bars indicate the regions of ECOP.
Based on Table~\ref{table:experiment_ECOP_satvis}, we observe that NRHO achieves the greatest at least one satellite visibility, which is $99.9\%$ of the total time, and also the greatest at least four satellite visibility, which is $92.9\%$ of the total time. 
Furthermore, NRHO also exhibits the least maximum ECOP of only $420$~\si{s}, while the other orbit types experience ECOP of at least $2880$~\si{s}. 
Intuitively, these observations related to NRHO seems reasonable, given that NRHO operates at high altitudes ranging between $4500-700000$~\si{km} above the Moon's surface, and thus experiences fewer occultations from Earth and the Moon. 
Comparing Figs.~\ref{fig:elfo_subsatvis},~\ref{fig:nrho_subsatvis},~\ref{fig:llo_subsatvis} and~\ref{fig:pco_subsatvis}, we observe that LLO, which has the lowest altitude of only $100$~\si{km}, exhibits the shortest time spacing between consecutive regions of ECOP. 
%From Figs.~\ref{fig:LLO_fullsatvis},~\ref{fig:LLO_fullsatvis} and~\ref{fig:elfo3_fullsatvis}, we observe that ELFO~\#1, which has the lowest altitude and, hence, the lowest orbital period, exhibits five occurrences of maximum ECOP regions~(duration of $3060~$s), while only one occurrence of maximum ECOP is observed for ELFO~\#2 and ELFO~\#3 in an experiment duration of $2$ months.
\begin{table}[H]
\centering
\caption{Comparison analysis across different orbit types, where NRHO exhibits the least maximum ECOP as well as the greatest visibility of both at least one and at least four Earth-GPS satellites.}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Orbit Type\\ \end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Max ECOP (\si{s})\\ \end{tabular}}} & \multicolumn{2}{c|}{\textbf{Satellite Visibility (\%)}} \\ \cline{3-4} 
 &  & \textbf{$\geq 1$} & \textbf{$\geq 4$} \\ \hline
\textbf{ELFO} & 3360 & 99.2 & 92.1 \\ \hline %99.1997 & 92.0755
\textbf{NRHO} & \textbf{420} & \textbf{99.9} & \textbf{93.0} \\ \hline
\textbf{LLO} & 2880 & 61.5 & 55.6 \\ \hline
\textbf{PCO} & 3900 & 98.1 & 90.8 \\ \hline
\end{tabular}
\label{table:experiment_ECOP_satvis}
\end{table}

\subsection{Across Clock Types: Variation in RMS Timing Errors}
To analyze the trade-off among different case studies of the orbit and the clock types, we compare the RMS estimation error in clock bias and drift in Table~\ref{table:rmse_timing_errors}. 
Intuitively, RMS timing error provides insights regarding the component of lunar UERE metric that represents the error due to broadcast clock. 
For a given Microchip CSAC, whose low SWaP characteristics were reported earlier in Table~\ref{table:LNSSsatclocks}, Fig.~\ref{fig:experiment_rmse_timing_errors} provides an illustration of the variation in timing errors across the four orbit types, namely ELFO, NRHO, LLO and PCO. 
In Fig.~\ref{fig:experiment_rmse_timing_errors}, we follow the same color coding as that in Figs.~\ref{fig:LNSSsatelliteThreeOrbitTypes} and~\ref{fig:LNSSsatelliteNRHO} to denote different orbit types, with ELFO indicated in orange, NRHO in green, LLO in magenta and PCO in blue. 

For a given Microchip CSAC onboard an LNSS satellite, we observe that the three orbit types, namely ELFO, NRHO and PCO, demonstrate a comparable RMS timing error of $<0.0282$~\si{\mu s} in clock bias and $<0.0444$~\si{ns/s} in clock drift, while the case study based on LLO shows a higher RMS error in clock bias of $0.0604$~\si{\mu s}.
This observation implies that the RMS timing error not only depends on the least maximum ECOP and the greatest satellite visibility but also on orbital parameters, namely eccentricity, inclination and altitude, that govern the geometric configuration between the Earth-GPS and LNSS.
We also observe that as the SWaP and the timing stability of the onboard clock increases, the variation in RMS error across orbit types becomes less significant, wherein the RMS error in clock bias and drift for DSAC are $<0.0021$~\si{\mu s} and $<4.8426\times 10^{-5}$~\si{ns/s}, respectively. 

\begin{table}[H]
\centering
\caption{Comparison analysis across different orbit types, where NRHO exhibits the least maximum ECOP as well as the greatest visibility of both at least one and at least four Earth-GPS satellites.}
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}RMS Timing Error \\ in Clock Type\end{tabular}}} & \textbf{ELFO} & \textbf{NRHO} & \textbf{LLO} & \textbf{PCO} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Microchip\\ CSAC\end{tabular}}}} & \textbf{Bias (\si{\mu s})} & 0.0264 & 0.0245 & 0.0604 & 0.0282 \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \textbf{Drift (\si{ns/s})} & 0.0442 & 0.0439 & 0.0467 & 0.0444 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Microchip \\ MAC\end{tabular}}}} & \textbf{Bias (\si{\mu s})} & 0.0128 & 0.0125 & 0.0184 & 0.0128 \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \textbf{Drift (\si{ns/s})} & 0.0078 & 0.0078 & 0.0080 & 0.0078 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}SRS\\ PRS-10\end{tabular}}}} & \textbf{Bias (\si{\mu s})} & 0.0102 & 0.0100 & 0.0134 & 0.0101 \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \textbf{Drift (\si{ns/s})} & 0.0042 & 0.0042 & 0.0043 & 0.0042 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Excelitas\\ RAFS\end{tabular}}}} & \textbf{Bias (\si{\mu s})} & 0.0066 & 0.0067 & 0.0079 & 0.0065 \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \textbf{Drift (\si{ns/s})} & 0.0012 & 0.0012 & 0.0012 & 0.0012 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NASA's\\ DSAC\end{tabular}}}} & \textbf{Bias (\si{\mu s})} & \textbf{0.0021} & \textbf{0.0023} & \textbf{0.0024} & \textbf{0.0021} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \textbf{Drift (\si{ns/s})} & \textbf{4.6554$\times 10^{-5}$} & \textbf{4.8426$\times 10^{-5}$} & \textbf{4.7114$\times 10^{-5}$} & \textbf{4.6032$\times 10^{-5}$} \\ \hline
\end{tabular}
\label{table:rmse_timing_errors}
\end{table}

\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/csac_FullfigureClockBias_OneClockMultipleOrbits.png}
		\caption{Clock bias error for entire experiment duration}
	\end{subfigure}	
	\hspace{2mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/csac_SubfigureClockBias_OneClockMultipleOrbits.png}
		\caption{Clock bias error for a smaller time segment}
	\end{subfigure}
	\vfill
	\vspace{5mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/csac_FullfigureClockDrift_OneClockMultipleOrbits.png}
		\caption{Clock drift error for entire duration}
	\end{subfigure}
	\hspace{1mm}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/csac_SubfigureClockDrift_OneClockMultipleOrbits.png}
		\caption{Clock drift error for a smaller time segment}
	\end{subfigure}	
	\caption{Comparison of estimation errors in clock bias and drift across different orbit types with an onboard Microchip CSAC, where ELFO is indicated in orange, NRHO in green, LLO in magenta, and PCO in blue; a) and c) demonstrate the errors in clock bias and clock drift for the entire experiment duration, respectively, while b) and d) demonstrate the zoomed-in errors in clock bias and clock drift for a smaller time segment of $2$~days. We observe that the three orbit types, namely ELFO, NRHO and PCO, demonstrate a comparable RMS timing error of $<0.0282$~\si{\mu s} in clock bias and $<0.0444$~\si{ns/s} in clock drift, while the LLO exhibits slightly higher RMS error in clock bias of $0.0604$~\si{\mu s}.}
	\label{fig:experiment_rmse_timing_errors}
\end{figure}

 


\subsection{Comparison Analysis of Lunar UERE}
We determine the lunar UERE metric across various case studies to compare the trade-off between different design considerations related to the onboard clock and the orbit type. 
As mentioned previously in Section~\ref{ssec:algorithm_lunarURE}, an important component of the lunar UERE is the broadcast clock error, which corresponds to the estimated RMS clock bias error associated with our proposed time-transfer technique. 
With pre-specified RMS values of other error sources listed earlier in Section~\ref{sec:implementation_details}, Fig.~\ref{fig:LunarUEREmetric} demonstrates the variation of lunar UERE metric across case studies conducted. 

We validate that our proposed time-transfer achieves a low lunar UERE of $<10$~\si{m} for most case studies except the one involving the LLO and the Microchip CSAC, which exhibits a value of $18.4$~\si{m}.
Furthermore, we observe that the estimated lunar UERE is comparable in order of magnitude to that of Earth-GPS, thus validating our LNSS design which utilizes time-transfer from Earth-GPS to lower the SWaP requirements of the onboard clock. 
These observations imply that, if the desired lunar UERE to be maintained by an LNSS satellite is, for instance, $<10$~\si{m} at all times, we can easily opt for an onboard clock that falls in the lower end of the SWaP spectrum, such as Microchip CSAC~$(17$~\si{cm^3}$\cdot 0.0035$~\si{kg}$\cdot 0.12$~\si{W}$)$ or Microchip MAC~$(50$~\si{cm^3}$\cdot 0.0084$~\si{kg}$\cdot 0.5$~\si{W}$)$, instead of a high-SWaP clock, such as Excelitas RAFS or NASA's DSAC.
Given a desired lunar UERE to maintain, we can also wisely choose the orbit type that is easy to maintain and has a longer lifespan, such as LLO, PCO or ELFO, over the more complex NRHO that requires constant station-keeping maneuvers to maintain stability.   
Furthermore, for future investigations, we observe the potential for a heterogenous, SmallSat-based lunar PNT constellation, wherein we can choose the grade of the onboard clock based on the orbit of each LNSS satellite to satisfy a desired lunar UERE.
For instance, to maintain a desired lunar UERE of $<5$~\si{m}, we observe from Fig.~\ref{fig:LunarUEREmetric} that we can design a heterogenous LNSS constellation based in ELFO and LLO, wherein the satellites in LLO can be equipped with a PRS-10 clock while the ones in ELFO can be equipped with a lower-SWaP Microchip MAC.  
\begin{figure}[H]
\centering
\includegraphics[width=0.45\textwidth]{figures/lunarUERE_AcrossClocks.png}
\caption{Comparison analysis of lunar UERE metric across five clock types and four orbit types. The estimated lunar UERE across all case studies has a comparable order of magnitude to that of the Earth-GPS UERE.}
\label{fig:LunarUEREmetric}
\end{figure}

==> old_sections/introduction.tex <==
% \begin{figure}[H]
% 	\setlength{\belowcaptionskip}{-4pt}
% 	\centering
% 	\includegraphics[width=0.6\textwidth]{figures/cn0-07-svn-48.png}
% 	\caption{Illustration of the received $\cno$ simulated in STK from PRN $7$ of the Earth-GPS constellation to an LNSS satellite in ELFO~\#1 at an altitude of $6541.5~$km. We observe intermittent availability of the Earth-GPS satellite signal, i.e., when $\cno$ is greater than the pre-specified threshold of $15~$dB-Hz, which is denoted by black dashed line. }
% 	\label{fig:receivedCN0value}
% \end{figure}
%% Copying this figure here, since i thought maybe it makes more sense in motivation?

\newpage

\section{Introduction}\label{sec:intro}

Over a half century since the end of the Apollo program, NASA will return humans to the Moon. 
In the coming decade, through the Artemis missions, National Aeronautics and Space Administration~(NASA) will land the first woman and person of color on the lunar south pole~\cite{smith2020artemis}. 
Additionally, many space agencies are participating in an international effort to establish a sustainable human presence on the Moon, which serves as a crucial platform to support future deep space exploration~\cite{laurini2014global}. 
Indeed, we are entering a second space race, with international space agencies planning over forty lunar missions in the next decade~\cite{tai2020ioag} and with crucial involvement from the commercial space industry companies, including SpaceX and Blue Origin.
To support the increasing plans for crewed and robotic missions, future lunar missions will require access to reliable and precise Position, Navigation, and Timing (PNT) services. 

% Paragraph 1: emerging space race, rush to return to the Moon
% \begin{itemize}
%     \item After over fifty years since the end of the Apollo program, NASA seeks to return humans to the Moon.
%     \item Indeed, through the Artemis missions in the coming decade, NASA plans to land the first woman and the first person of color on the lunar south pole 
%     \item Important to return to the Moon -- crucial stepping stone for future deep space missions, including...
%     \item International goal: establish a sustainable human presence on the Moon~\cite{laurini2014global}
%     \item Correspondingly, we are entering a second space race, with international space agencies planning over forty lunar missions planned over the next decade~\cite{tai2020ioag} and with additional lunar missions planned by private sector companies, including SpaceX and Blue Origin.
% \end{itemize}


Current state-of-the-art techniques for providing deep space PNT include Terrain Relative Navigation~(TRN) with onboard camera sensors~\cite{downes2020deep,conte2009vision,steiner2015graph,thornton2003radiometric,lanyi2008radiometric,broschart2017optical} and radio navigation using the Deep Space Network~(DSN)~\cite{mudgway2001uplink}. 
In particular, TRN techniques rely on matching images taken from a camera sensor with an onboard database of distinctive land features in space. 
TRN was recently utilized to perform precise landing for the Mars Perseverance rover in February of 2021~\cite{bolles2020terrain}.
However, vision-based navigation techniques perform poorly in areas with low lighting, including permanently shadowed regions, both of which are key sites of interest for the upcoming Artemis missions.
Furthermore, TRN requires extensive memory and computation resources onboard the spacecraft~\cite{dubois2009testing}.

Radio navigation with the DSN involves sending precisely timed signals between the spacecraft and ground monitoring stations on Earth.
As a result, these techniques require a direct, line-of-sight view of the terrestrial ground stations, which is unavailable in the polar craters and on the far side of the Moon.
Furthermore, this approach requires scheduling communication links with the DSN, which is expected to be overburdened with increasing communication demands from the wave of upcoming space missions~\cite{foust2021increasing}.
Additionally, due to the communication scheduling requirements as well as the distance between the Moon and DSN, satisfying the precise and real-time lunar navigation becomes challenging. %\tara{need to check sentence}.

To address these challenges, the NASA Goddard Space Flight Center (GSFC) and the European Space Agency~(ESA) have conceptualized GPS-like satellite constellations, named LunaNet~\cite{israel2020lunanet} and Moonlight~\cite{cozzens2021moonlight} respectively, around the Moon. %\tara{need to spell out NASA/ESA if not done already?} \ramya{did this-wrote the full forms of both!}
These lunar constellations will assist in the overarching effort of establishing a sustainable human presence on the Moon, by providing PNT and communication services to lunar users.
In particular, in the next decade, these initiatives seek to satisfy needs expressed by the Global Exploration community, with a targeted position accuracy of less than $50$~\si{m}~\cite{cozzens2021moonlight}.
However, because these lunar constellation initiatives are in the preliminary design phases, many key design considerations still need to be finalized, including the satellite orbits, payload, and onboard clock.

Designing a Lunar Navigation Satellite System (LNSS) involves unique challenges, which lead to different key design considerations and limitations as compared to the legacy Earth-GPS system:
\begin{enumerate}
    \item Limited size of LNSS satellites. 
    Indeed, NASA GSFC has expressed interest in using a SmallSat platform for the future LunaNet constellation to allow for cost-effective and rapid deployment~\cite{israel2020lunanet,israel2020lunanet_ssc}. 
    However, a smaller satellite platform limits its payload capacity, including the Size, Weight, and Power (SWaP) of the onboard clock.
    Given that lower SWaP clocks tend to have worse timing stabilities~\cite{schmittberger2020review}, the limitation on clock SWaP directly affects the timing precision and, thus, the ranging precision of the PNT measurements the LNSS satelite provides users.
    \item Limited ability to monitor for LNSS satellites. Given that a limited number of ground monitoring stations can be established on the Moon and that resources on Earth for monitoring the lunar constellation are limited, it is desirable for the LNSS satellites to require less maintenance, including fewer station-keeping maneuvers and clock correction maintenance.
    \item Increased orbital perturbations in lunar environment. Because the Moon has a highly non-uniform distribution~\cite{melosh2013origin}, its gravitation field is more anisotropic as compared to that of Earth's. In addition to these orbital perturbations, Earth's gravity can significantly impact satellites in high-altitude lunar orbits, thereby limiting the set of feasible and stable lunar orbits. %\tara{should we keep this? since we were previously using this to justify using an ELFO}
    % \item Limited financial investment. In contrast with the legacy Earth-GPS system, the LNSS will be significantly more limited in financial budget, thereby leading to fewer overall resources to establish and maintain the system.
\end{enumerate}
%Given the unique challenges for designing a PNT constellation in the lunar environment, in our prior work~\cite{bhamidipati2021design}, we investigated the potential of leveraging the established, legacy Earth-GPS, which is equipped with higher grade atomic clocks and an extensive ground monitoring network for continuous maintenance.
Given these challenges for designing a PNT constellation in the lunar environment, one may consider the potential in leveraging the nearby, existing Earth's legacy GPS system, which is equipped with higher grade atomic clocks and an extensive ground monitoring network for continuous maintenance.
At lunar distances of about $385000$~\si{km}, the Earth-GPS signal is significantly attenuated, and the Earth-GPS satellites directed toward the Earth are largely occluded by the Earth and often the Moon, leaving only small, unoccluded parts of the main lobe the side lobes, as shown in Fig.~\ref{fig:EarthGPSvisibility}. 
Despite these challenges, however, Earth-GPS signal sidelobes have been previously used to obtain a position estimate in space at distances about one-fifth of the way to the Moon~\cite{winternitz2017global} %\tara{the Winterniz 2017 paper says one-fifth, but read in ESA article ``Galileo will help Lunar Pathfinder navigate around Moon'' that it is about halfway, need to check}  
and several works have demonstrated the feasibility of using Earth-GPS at lunar distances~\cite{schonfeldt2020system,winternitz2019gps,cheung2020feasibility}.
NASA has additionally characterized the GPS antenna gain patterns at high elevation angles from boresight for space users~\cite{donaldson2020characterization} and has developed a spaceborne GPS receiver~\cite{winternitz2004navigator}, which will be tested on the lunar surface for the first time in 2023~\cite{insideGNSS2021luGRE,kraft2020luGRE}.
Additionally, in 2023, the ESA will launch the Lunar Pathfinder communication satellite to the Moon, which will utilize a spaceborne, high-sensitivity GPS receiver to provide a position fix for the first time in lunar orbit~\cite{esa2021pathfinder}.

To address the unique challenges for designing an LNSS, in our prior work~\cite{bhamidipati2021design}, we sought to harness the legacy Earth-GPS system to provide precise timing corrections to the newly conceptualized LNSS system, as depicted in Fig.~\ref{fig:proposedtimetransfer}. 
Our proposed time-transfer technique leverages intermittently available Earth-GPS signals to alleviate the cost and SWaP requirements of the onboard clocks and the need for additional ground infrastructure to maintain the LNSS services.
We further demonstrated that with our proposed method, we can achieve low lunar User Equivalent Range Error~(UERE) of less than $10$~\si{m} while alleviating the SWaP of the onboard clock by using a low-SWaP Chip Scale Atomic Clock~(CSAC) for a lunar satellite in Elliptical Lunar Frozen Orbit~(ELFO).
% However, given that many design choices still need to be finalize for the future SmallSat-based LNSS, in this work, we analyze the trade-off between design considerations of the onboard clock and the orbit type for an LNSS conducting time-transfer from Earth-GPS.
% Specifically, we conduct various case studies with different grades of onboard, low-SWaP clocks and various previously studied lunar orbit types, including the Elliptical Lunar Frozen Orbit (ELFO), Low Lunar Orbit (LLO), Prograde Circular Orbit (PCO), and Near-Rectilinear Halo Orbit (NRHO). 

Given that many design choices still need to be finalize for the future SmallSat-based LNSS, including the grade of the onboard clock and the orbit type, in this work, we extend our prior work~\cite{bhamidipati2021design} to analyze the LNSS system performance using our time-transfer architecture from Earth-GPS under various case studies.
Specifically, we conduct case studies with different grades of onboard, low-SWaP clocks and various previously studied lunar orbit types, including the ELFO, Low Lunar Orbit (LLO), Prograde Circular Orbit (PCO), and Near-Rectilinear Halo Orbit (NRHO). 
For a given LNSS satellite orbit, we examine an Earth-GPS Continual Outage Period (ECOP) metric to analyze the visibility effects of Earth-GPS on the timing stability of the onboard clock. 
We further estimate the lunar UERE metric to characterize the accuracy of the ranging signals transmitted from the LNSS satellite. 
Through our analysis, we illustrate the trade-off between the different design considerations of the onboard clock and the orbit type for an LNSS leveraging Earth-GPS time-transfer.
We additionally observe across the various case studies that with our time-transfer architecture, the LNSS can achieve comparable performance as that of the legacy Earth-GPS, even while using a low-SWaP onboard clock.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/receivedCN0.png}
\caption{Earth-GPS signals at lunar distances are received from the side lobes and small parts of the main lobes. 
The received $\cno$ depends on the transmit power and transmit antenna gain pattern of the Earth-GPS satellite, occultation from the Earth and the Moon, and free-space path loss.}
\label{fig:EarthGPSvisibility}
\vspace{-3mm}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/Architecture4.png}
\caption{Architecture of our proposed time-transfer from Earth-GPS~\cite{bhamidipati2021design}, which utilizes intermittently available Earth-GPS signals to correct the lower grade clocks onboard the LNSS satellite.}
\label{fig:proposedtimetransfer}
\vspace{-3mm}
\end{figure}


% We propose the design of a SmallSat-based LNSS with time-transfer from Earth-GPS, wherein the LNSS satellites will listen to signals already broadcast by the Earth-GPS and process those signals to estimate timing corrections.
% An illustration of our proposed time-transfer technique is shown in Fig.~\ref{fig:proposedtimetransfer}. 
% We design a timing filter that corrects the lower grade clock onboard an LNSS satellite when Earth-GPS signals are available, and when Earth-GPS signals are unavailable, we propagate these clock estimates forward in time. 
% We also develop an Earth-GPS Continual Outage Period (ECOP) metric to analyze the visibility effects of Earth-GPS on the timing stability of the onboard clock.
% Our proposed Earth-GPS-to-LNSS time-transfer technique alleviates requirements with regards to timing stability and, correspondingly, the SWaP of the onboard clocks. 
% Additionally, our design leverages Earth-GPS signals, thereby eliminating the need for additional ground infrastructure to maintain the LNSS services. 
% Furthermore, our design facilitates navigation across the complete lunar landscape with the LNSS constellation. 

\subsection{Key Contributions} 
The key contributions of our paper are listed as follows:
\begin{enumerate}
    \item We design case studies with different onboard clocks and orbit types to analyze the trade-offs in designing an LNSS with time-transfer from Earth-GPS.
    In particular, we investigate five clock types with diverse SWaP characteristics that range from a low-SWaP CSAC to a high-SWaP Deep Space Atomic Clock~(DSAC)~\cite{ely2018using, ely2014advancing} developed by NASA. 
    In our case study analysis, we also investigate four previously studied types of lunar orbits which include ELFO, NRHO, LLO and PCO. 
    \item We perform a comparison analysis across various case studies by investigating the associated RMS timing errors, which are in-turn governed by the duration for which no Earth-GPS satellites are available~(ECOP metric) and the geometric configuration between the Earth-GPS constellation and the LNSS satellite.  
    \item We evaluate the lunar UERE metric for each case study and demonstrate comparable ranging precision as that of the legacy Earth-GPS, even while using a low-SWaP onboard clock. 
\end{enumerate}
% The key contributions of our SmallSats-based Earth-GPS-to-LNSS time-transfer technique are as follows: 
% \begin{enumerate}
%     \item We develop a timing filter, based on a Kalman filter framework, to update the lower grade clock onboard an LNSS satellite using intermittently available Earth-GPS signals. 
%     \item We devise a lunar User Equivalent Range Error (UERE) metric to characterize the ranging accuracy of an LNSS satellite. For a given orbit and an onboard clock, the lunar UERE depends on the Root-Mean-Square~(RMS) timing error estimated using our proposed time-transfer technique. This is because any timing error is directly reflected in the ranging accuracy. 
%     \item We validate our time-transfer using simulations of an LNSS satellite in Elliptical Lunar Frozen Orbit (ELFO) with an onboard Chip Scale Atomic Clock (CSAC). We also perform sensitivity analysis across different ELFO configurations, by varying Keplarian parameters, in terms of various metrics, such as maximum ECOP, timing errors and lunar UERE.
% \end{enumerate}

%\tara{should we have a key contributions section? is it necessary? was a bit at a loss for what to write}
%\ramya{sure! I can write this part when I am writing the conclusions. thanks for leaving a message here!}
%\tara{oh okay cool lol, I guess I feel like I wrote some things in the previous paragraph which describe what this work does.. but I didn't really feel like any of them were particularly \textit{new} contributions, so I felt a bit unsure if we even needed an additional separate section for this}
%\ramya{yeah, I agree. I think I have conclusions/observations from experiments, not sure if they can be called contributions? We can perhaps discussion this in the afternoon. Maybe we can repeat some of them from ION paper, and some new ones can focus more on case study validation aspects}

%\tara{need to update this..} \ramya{done!}
The rest of the paper is organized as follows.
Section~\ref{sec:proposed_time_transfer_technique} summarizes our proposed time-transfer technique from Earth-GPS to LNSS. 
Section~\ref{sec:simulation_modeling} describes our high-fidelity lunar simulation setup that involves modeling the onboard clocks and the orbit types chosen for our case study. 
Section~\ref{sec:experiment_results} discusses the implementation and implications of our case study analysis. 
Section~\ref{sec:conclusion} provides concluding remarks.

==> old_sections/method.tex <==
\section{Our Proposed Time-Transfer from Earth-GPS to LNSS} \label{sec:proposed_time_transfer_technique}

To perform time-transfer from Earth-GPS, we consider an LNSS satellite equipped with a spaceborne Earth-GPS receiver and a lower grade clock that can provide short-term timing stability.
From our prior work~\cite{bhamidipati2021design}, we designed a timing Kalman filter~\cite{krawinkel2016benefits, martoccia1998gps} to update the LNSS satellite clock with the intermittently available Earth-GPS signals and maintain precise timing.
In Section~\ref{ssec:filter}, we describe our Kalman filter-based Earth-GPS-to-LNSS time-transfer technique proposed in our prior work, and in Section~\ref{ssec:algorithm_lunarURE} we discuss the error components that make up the lunar UERE metric.

\subsection{Clock Estimation via Timing Filter}\label{ssec:filter}
The architecture of our timing Kalman filter to perform time-transfer with the intermittently available Earth-GPS signals~\cite{bhamidipati2021design} is depicted in Fig.~\ref{fig:high_level_arch}. 
Our filter maintains the LNSS clock estimate with time and measurement updates, with the use of position and velocity aiding from available ephemeris information for the LNSS satellite.
At each time step, we analyze the received carrier-to-noise density ratio~$\cno$ to check if any Earth-GPS signals are visible.
If no Earth-GPS signals are visible, we only perform a time update, based on the clock error propagation model, as discussed further in Section~\ref{sec:timeupdate}, whereas if any Earth-GPS signals are available, we additionally perform a measurement update, as discussed further in Section~\ref{sec:measurementupdate}. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/v2Flowchart.png}
    \caption{High-level architecture of our timing filter~\cite{bhamidipati2021design}. The LNSS satellite, equipped with a spaceborne Earth-GPS receiver and a lower grade clock, utilizes its position and velocity information to obtain residual pseudorange and pseudorange rate measurements from each visible Earth-GPS satellite. When Earth-GPS signals are available, we additionally correct the clock estimates of bias and drift.}
    \label{fig:high_level_arch}
\end{figure}

The timing state vector at each time step $t$ is defined as
\begin{align}
    \state\tidx{t} \coloneqq \begin{bmatrix} \clkbias\tidx{t} & \clkbiasrate\tidx{t} \end{bmatrix}^{\top}, \label{eq:statevector}
\end{align}
where $\clkbias\tidx{t}$ is the clock bias state in \si{m} and $\clkbiasrate\tidx{t}$ is the clock drift in \si{ms^{-1}}, with units converted from the timing domain through multiplication by the speed of light $\speedoflight=299792458$~m/s.

\subsubsection{Time Update Step} \label{sec:timeupdate}
At each time step, the timing filter propagates the state vector in Eq.~\eqref{eq:statevector} according to the following first-order random process:
\begin{align}
    \pred{\state}\tidx{t} &= A\state\tidx{t-1}, \label{eq:pred_state} \\
    \pred{\cov}\tidx{t} &= A\cov\tidx{t-1} A^\top + Q, \label{eq:pred_cov} \\
    A &\coloneqq \begin{bmatrix} 1 & \sampinterval \\ 0 & 1 \end{bmatrix}
\end{align}
where $\pred{\state}\tidx{t}$ is the predicted state, $\pred{\cov}\tidx{t}$ is the error covariance of the propagated state, $\sampinterval$ is the filter update time interval, and we define the process noise covariance $Q$ as
\begin{align}
    Q &\coloneqq \speedoflight^2\,\begin{bmatrix} \frac{h_0}{2}\sampinterval + 2 h_{-1} \sampinterval^2 + \frac{2}{3} \pi^2 h_{-2}^2 \sampinterval^3 & h_{-1} \sampinterval + \pi^2 h_{-2}\sampinterval^2 \\
    h_{-1} \sampinterval + \pi^2 h_{-2} \sampinterval^2 & \frac{h_0}{2\sampinterval} + 4h_{-1} + \frac{8}{3} \pi^2 h_{-2} \sampinterval
    \end{bmatrix} \label{eq:def_propcov}
\end{align}
where the $h_\alpha$ terms are the power spectral density coefficients from the clock Allan deviation plot~\cite{krawinkel2016benefits}, which reflect the short-term and long-term stability of the onboard clock~\cite{van1984relationship}.

\subsubsection{Measurement Update Step} \label{sec:measurementupdate}
When Earth-GPS satellite measurements are available, we perform a measurement update of the timing state vector. 
Because the LNSS ephemeris parameters require less frequent updates as compared to the timing state vector of the lower grade onboard clock, we assume that the ephemeris is maintained outside of the proposed timing filter, such as by an onboard orbit determination module~\cite{erdogan2009near}.
As a result, with knowledge of the LNSS satellite position and velocity, we determine the expected pseudorange and pseudorange rates from the visible Earth-GPS satellites to form a measurement vector of residuals:
\begin{align}
    \meas\tidx{t} \coloneqq \begin{bmatrix} \prngres\tidx{t}\satidx{1} & \cdots & \prngres\tidx{t}\satidx{N\tidx{t}} & \prngrateres\tidx{t}\satidx{1} & \cdots & \prngrateres\tidx{t}\satidx{N\tidx{t}} \end{bmatrix}^{\top}, \label{eq:res_meas}
\end{align}
where $N\tidx{t}$ is the number of visible satellites at time $t$, and $\prngres\tidx{t}\satidx{i}$ and $\prngrateres\tidx{t}\satidx{i}$ are the pseudorange and pseudorange rate residuals, respectively, from satellite $i$, which are formed via the expressions:
\begin{align}
    \prngres\tidx{t}\satidx{i} &\coloneqq \prngmeas\tidx{t}\satidx{i} - \prngexp\tidx{t}\satidx{i}, \\
    \prngrateres\tidx{t}\satidx{i} &\coloneqq \prngratemeas\tidx{t}\satidx{i} - \prngrateexp\tidx{t}\satidx{i},
\end{align}
where $\prngmeas\tidx{t}\satidx{i}$ and $\prngratemeas\tidx{t}\satidx{i}$ are the received pseudorange and pseudorange rate measurements, respectively.
Analogously, $\prngexp\tidx{t}\satidx{i}$ and $\prngrateexp\tidx{t}\satidx{i}$ are the expected pseudorange and pseudorange rate measurements, respectively, from Earth-GPS satellite~$i$ at time step $t$, computed from the LNSS satellite and Earth-GPS satellite position and velocity.

From the residual measurement vector in Eq.~\eqref{eq:res_meas}, we apply corrections to the predicted timing state via the following standard Kalman filter expressions to obtain the updated state $\crct{\state}\tidx{t}$ and covariance $\crct{\cov}\tidx{t}$:
\begin{align}
    \kalmangain\tidx{t} &\coloneqq \pred{\cov}\tidx{t} \measmat^\top \left(\measmat \pred{\cov}\tidx{t} \measmat^\top + \meascov\tidx{t} \right)^{-1}, \\
    \crct{\state}\tidx{t} &= \pred{\state}\tidx{t} + \kalmangain\tidx{t} \left( \meas\tidx{t} - \measmat \pred{\state}\tidx{t} \right), \\
    \crct{\cov}\tidx{t} &= \left( I_2 - \kalmangain\tidx{t} \measmat\right)\pred{\cov}\tidx{t}, 
\end{align}
where $\kalmangain\tidx{t}$ is the Kalman gain matrix, $\meascov\tidx{t}$ is the measurement noise covariance, $I_{a}$ denotes the identity matrix of size~$a\times a$, and $C\in \mathbb{R}^{2N\times 2}$ is the measurement model associated with pseudorange and pseudorange rate residuals, defined as:
\begin{align}
    \measmat &= \begin{bmatrix} 1_{N\times 1} & 0_{N\times 1} \\
    0_{N\times 1} & 1_{N\times 1} \end{bmatrix}
\end{align} 
where $1_{a\times b}$ and $0_{a\times b}$ represent size $a \times b$ matrices of ones and zeros, respectively.


We model $\meascov\tidx{t}$ as a diagonal matrix:
\begin{align} \label{eq:measurementnoisecovariance}
    \meascov\tidx{t} &= 
    \text{diag}\left(
    \big(\varprng\tidx{t}\big)\satidx{1},
    \cdots, \big(\varprng\tidx{t}\big)\satidx{N\tidx{t}},
    \big(\varprngrate\tidx{t}\big)\satidx{1},
    \cdots,
    \big(\varprngrate\tidx{t}\big)\satidx{N\tidx{t}} 
    \right),
\end{align}
where  $\varprng\tidx{t}\satidx{i}$ is the pseudorange residual measurement variance in \si{m^2} and $\varprngrate\tidx{t}\satidx{i}$ is the pseudorange rate residual measurement variance in \si{m^2s^{-2}} from the $i^{\text{th}}$ Earth-GPS satellite at time $t$.
We model both variance terms as being time-dependent due to the fluctuations in the $\cno$ of each received Earth-GPS signal, which relates to the tracking errors of the receiver Delay Lock Loops~(DLLs) and Phase Lock Loops~(PLLs).
In particular, for the pseudorange residual measurement variance, we model the pseudorange residual measurement variance as~\cite{bhamidipati2021design}:
\begin{align} 
    \big(\varprng\tidx{t}\big)\satidx{i} &= \big(\vardll\tidx{t}\big)\satidx{i} + \varuereearth + \varlunareph, \label{eq:pseudorangecov}
\end{align}
where $\vardll\tidx{t}\satidx{i}$ is the variance in \si{m^2} in the $i^\text{th}$ Earth-GPS satellite due to the error in a non-coherent power DLL discriminator, which we model in our prior work~\cite{bhamidipati2021design} based on the formulation from~\cite{kaplan2017understanding} and used in~\cite{capuano2015feasibility,capuano2016gnss}.
Additionally, $\varuereearth$ is the variance to the space and control segment of the Earth-GPS system UERE, which include the errors in the broadcast clock and ephemeris~\cite{kaplan2017understanding}, and $\varlunareph$ is the measurement variance component due to the uncertainty in the LNSS satellite ephemeris.

From our prior work~\cite{bhamidipati2021design}, we additionally model the pseudorange rate residual measurement variance $\big(\varprngrate\tidx{t}\big)\satidx{i}$ according to the receiver PLL tracking error of the signal from the $i^{\text{th}}$ Earth-GPS satellite~\cite{borio2011doppler, capuano2016gnss}.



\subsection{Formulation of the Lunar UERE Metric} \label{ssec:algorithm_lunarURE}

In our prior work~\cite{bhamidipati2021design}, we formulated a lunar UERE metric to characterize the accuracy of the LNSS ranging signals for lunar users.
Table~\ref{tab:uere_earth_gps} outlines the ranging error components that make up the lunar UERE and compares them with the list of error components that constitute the Earth-GPS UERE for a single-frequency receiver~\cite{kaplan2017understanding}.
On the Moon, any atmospheric delays are minimal. Moreover, we also consider multipath effects experienced by users on the lunar surface to be negligible due to the lack of building infrastructure and foliage. 
As a result, the final lunar UERE can be computed in terms of four most significant error components as follows:
\begin{align}
    \stdueremoon = \sqrt{\stdlunarclk^2 +\stdlunargd^2+\stdlunareph^2+\stdlunarrec^2}
\end{align}
The errors due to the differential group delay~$\stdlunargd$ and the receiver noise~$\stdlunarrec$ will depend on the final LNSS signal structure and lunar user receiver.
In this work, we simulate how the LNSS clock error component~$\stdlunarclk$ differs for various clock types and lunar orbits and analyze the corresponding impact on the overall lunar UERE.
Note that, because the timing filter uses position aiding from the lunar satellite, the lunar ephemeris error~$\stdlunareph$ directly impacts the error in the pseudorange residual measurement received at the LNSS, as modeled in Eq.~\eqref{eq:pseudorangecov}, which will thus also affect the LNSS clock error~$\stdlunarclk$. 
%\tara{are we doing case studies with scaling the lunar? for current draft, will not mention anything yet} \ramya{I did not add this for now, couldn't decide what we can show differently based on results. Thought based on adaptive filter stuff we add later, we can modify this.}
\begin{table}[h]
\centering
\caption{Individual error components for the lunar UERE formulation~\cite{bhamidipati2021design}, which include errors due to the broadcast clock, differential group delay, broadcast ephemeris and receiver noise and resolution. Other components, namely atmospheric delays and multiplath effects, are considered to be negligible for the lunar environment. }
\begin{tabular}{|c|c|c|}
\hline
\textbf{LNSS segment} & \textbf{\begin{tabular}[c]{@{}c@{}}Error components\\ (based on Earth-GPS UERE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Lunar UERE \\ (based on $1\sigma$ error)\end{tabular}} \\ \hline
\multirow{3}{*}{\textbf{Space/Control}} & Broadcast clock &  $\stdlunarclk$\\ \cline{2-3} 
 & Differential group delay & $\stdlunargd$ \\ \cline{2-3} 
 & Broadcast ephemeris &  $\stdlunareph$\\ \hline
\multirow{4}{*}{\textbf{User}} & Ionospheric delay &  -\\ \cline{2-3} 
 & Tropospheric delay &  -\\ \cline{2-3} 
 & Receiver noise and resolution &  $\stdlunarrec$\\ \cline{2-3} 
 & Multipath effects &  - \\ \hline
\end{tabular}
\label{tab:uere_earth_gps}
\end{table}





\begin{comment}
\begin{table}[H]
    \centering
    \caption{Individual error components that comprise the Earth-GPS and the lunar UERE~\cite{kaplan2017understanding}. In contrast with the Earth-GPS, for the LNSS, the lunar environment will have little to no atmospheric effects and multipath effects. In this work, we simulate and analyze $\stdlunarclk$ using Earth-GPS time-transfer. We further assume equivalent values as Earth-GPS for $\stdlunargd$ and $\stdlunarrec$, while enlarging the ephemeris error by one order of magnitude in comparison to Earth-GPS, i.e. $\stdlunareph=3~$m. }
    \begin{tabular}{|r|c|c|c|c|}
        \hline 
        System segment & Error component & Earth-GPS $1\sigma$ error (m) & LNSS $1\sigma$ error (m) \\
        \hline
        space/control & broadcast clock & 0.4 & $\stdlunarclk$ \\
        & differential group delay & 0.15 & $\stdlunargd$ \\
        & broadcast ephemeris & 0.3 & $\stdlunareph$ \\
        \hline
        user & ionospheric delay & 7.0 & - \\
        & tropospheric delay & 0.2 & - \\
        & receiver noise and resolution & 0.1 & $\stdlunarrec$ \\
        & multipath effects & 0.2 & - \\
        \hline
    \end{tabular}
    \label{tab:uere_earth_gps}
\end{table}
\end{comment}

%In the lunar UERE metric, the errors due to the differential group delay, broadcast ephemeris and receiver noise, greatly depend on the final signal structure of the LNSS constellation. % and user LNSS receiver devices. 
%Indeed, multipath could certainly become a key source of error in regions of the Moon with greatly varying topography, such as near the edges of craters 





%the Earth-GPS and the lunar UERE~\cite{kaplan2017understanding}. In contrast with the Earth-GPS, for the LNSS, the lunar environment will have little to no atmospheric effects and multipath effects. In this work, we simulate and analyze $\stdlunarclk$ using Earth-GPS time-transfer. We further assume equivalent values as Earth-GPS for $\stdlunargd$ and $\stdlunarrec$, while enlarging the ephemeris error by one order of magnitude in comparison to Earth-GPS, i.e. $\stdlunareph=3~$m. 

%\ramya{same comment as earlier regarding implementation details. check my changes. I will add these commented parts later in simulation or implementation section. }


==> old_sections/misc.tex <==
After more than fifty years since the Apollo program, we are encountering a revived, second Space Race with international space agencies seeking to not only return humans to the Moon, but to further establish a sustainable human presence.
Correspondingly, NASA and the ESA have conceptualized the initial framework for a GPS-like constellation for the Moon, which will ensure uninterrupted navigation and communication services for future lunar missions.
For the future Lunar Satellite Navigation system~(LNSS), NASA expresses interest in using a SmallSat platform, due to its cost-effectiveness and its potential for rapid deployment; however, many design decisions still need to be finalized, including the lunar orbit, constellation, payload, and onboard clock.
Furthermore, designing a dedicated LNSS involves additional challenges, which are unique to the lunar environment, including limited payload capacity for the SmallSat platform, i.e. the Size, Weight, and Power (SWaP) of the onboard clock, limited lunar ground monitoring stations and limited financial investment as compared to the legacy Earth-GPS.

Given these unique challenges for the lunar environment, we propose the design of a SmallSat-based LNSS with an inexpensive, low-SWaP onboard clock, which harnesses the satellite signals from the well-established Earth-GPS constellation to maintain precise timing. 
In particular, we develop a timing filter to correct the lower grade onboard clock, while leveraging the intermittently available Earth-GPS signals.
Additionally, we devise a lunar User Equivalent Range Error (UERE) metric to characterize the ranging accuracy of an LNSS satellite.
We further validate our proposed time-transfer technique with simulations of an LNSS satellite in an Elliptical Lunar Frozen Orbit (ELFO) with an onboard Chip Scale Atomic Clock (CSAC), while analyzing the visibility effects of Earth-GPS, timing stability, and lunar UERE across different configurations of ELFOs.

==> old_sections/outline.tex <==
\section*{Outline Example}
\begin{outline}[enumerate]
\1 Thing 1
    \2 Subthing 1
    \2 Subthing 2
        \3 Subsubthing 1
        \3 Subsubthing 2

\1 Thing 2   
\end{outline}

==> old_sections/outline_IONGNSS+.tex <==
\section{Introduction}
\begin{outline}[enumerate]
\1 Second space race / Motivation to return moon
    \2 Artemis mission
    \2 International goal for sustainable human presence on moon
    \2 60 upcoming mission...
    \2 South pole is a key interest region? (optional)

\1 Need for PNT for these missions
    \2 Near-term mission goals, need PNT for these missions
    \2 Earth has GPS
    \2 Can we have a GPS-like system for Moon?
        \3 In fact, NASA has lunaNet constellation. Interest in smallsats-> cost effectiveness and rapid deployment. 
        \3 ESA planning to develop Moonlight (within next 10 years) to provide an unprecedented target accuracy of 100 meters for upcoming lunar navigation
    
\1 Questions we need to answer on how satellite navigation is different on Moon and what are its challenges? 
    \2 Given limited payload/SWaP capability of small satellite configuration and limited financial investment / ground monitoring stations as compared to GPS (terrestrial, military asset), also need to be mindful of the challenges unique to lunar case/environment: less payload capacity / smaller satellites, less cost, less infrastructure for ground stations --> 
        \3 Given the limited ground infrastructure for the lunar satellites, one potential orbit being investigated for lunar PNT is ELFO due to its highly stable behavior and because it requires less station-keeping --cite ESA study. 
        \3 Given less payload capacity / smaller satellites, the future lunar satellite constellation will also be limited in the SWaP (Size, Weight, and Power) for the on-board clock 
    \2 Given these challenges, can we harness the Earth-GPS, which is a established system, to alleviate/address some of these challenges while designing LNSS (from clock perspective).  

\1 Leveraging Earth-GPS on the Moon. 
    \2 Is this possible since transmit antenna points towards the Earth because of which, main-lobe is occluded by Earth and Moon? Will the GPS signals be strong enough to navigate with at lunar distances?
    \2 Yes, it is possible. Many studies like NASA Navigator, ESA study analyzed the visibility of GPS signals at lunar distances. 
    \2 NASA ACE experiment also characterized the side-lobe performance and transmit antenna gain patterns.
    \2 Even though leveraging Earth-GPS signals is possible, Earth-GPS signals are not available at all times, only intermittently available with varying number of available measurements. 
    
\1 We design an LNSS propose a time-transfer technique from Earth-GPS to LNSS satellites.
    \2 We deal with intermittent availability via using timing-based kalman filter framework. 
    \2 We analyze the performance characteristics of our time-transfer framework 
        \3 with ELFO orbit and CSAC clock (no need to justify a second time?)
        \3 Different types of ELFO with different Keplarian parameters have been explored in literature
            \4 Varying visibility of GPS satellites %to leverage timing ability
            \4 Develop ECOP metric to analyze effect of visibility on timing stability
        \3 Even with CSAC, our time-transfer architecture can demonstrate reasonable timing accuracies / ranging accuracy for lunar navigation applications
    \2 We additionally develop a lunar URE metric to characterize the ranging accuracy for lunar PNT
        
\1 Key contributions
    \2 Time-transfer technique to harness Earth-GPS signals
    \2 Timing-based filter technique to account for the intermittently available Earth-GPS signals, and when none available, propagating the clock estimates forward in time
    \2 Formulate lunar URE metric based on RMS timing error from time-transfer technique. 
    \2 Demonstrate with ELFO and on-board CSAC the performance of our time-transfer algorithm. 
    \2 Sensitivity analysis for different considerations of ELFO in terms of max ECOP, timing errors and lunar URE. 
\end{outline}

\section{Proposed Algorithm - Tara}
\subsection{Time-transfer/Estimator}
\begin{outline}
\1 EKF -> estimator clock and estimator measurement models (time and measurement update)
\1 process noise and measurement covariance formulation (high-level, symbolic representation of error terms / URE terms)
\1 Tracking loop values used / citation
\end{outline}
\subsection{lunar URE}
\begin{outline}
\1 Error budget terms which are present and not compared to Earth
\1 RMS timing error is added to broadcast clock 
\1 lunar URE expression is sum of four terms
\end{outline}

%\section{Case studies: Orbits and Clocks - Ramya}

\section{GPS receiver/transmitter Modeling/ Simulation}

\subsection{High-level Assumptions}
\begin{outline}
\1 Simulate (via STK) the visibility and C/N0 of received GPS signals in lunar regime, while modeling the following (high-level):
    \2 Occlusion of Earth/Moon, antenna gain patterns, free space path loss, attitude / geometry
\1 Assumption: Directly model the pseudorange and Doppler residual. 
\1 Consider earth mask to remove Earth ionospheric and tropospheric effects
\1 Tracking times of 36 s considered.
\end{outline}

\subsection{Earth-GPS constellation}
\begin{outline}
\1 Antenna gain patterns from NASA ACE study. Block III modeling using same antenna patterns as block IIF. How <16 deg stuff are modeled to have the same constant value. Transmit powers from GPS antenna for L1 C/A -- also only using L1 C/A
\1 Almanac year of 2019/2020? Based on this almanac, 31 satellites -- not using PRN 14 because it is decommissioned (or STK doesn't have this info)?
\end{outline}

\subsection{Lunar satellite: ELFO orbit and clock}
Clock modeled using MATLAB and orbits using STK. 
\begin{outline}
\1 Clocks modeling: (Tara)
    \2 Explain limitation of payload -- why considering smaller clocks
    \2 SWaP of CSAC and why it is potentially useful for lunar applications.
    \2 True clock model based on time deviation --> Remarks about true vs estimator point out differences
\1 Orbit modeling: 
    \2 Start time of simulation considered
    \2 Keplarian orbit based modeling for ELFO -- HPOP to propagate
    \2 Orbit types and details of various ELFO --> altitude and keplarian orbits. Perhaps orbit characteristics and why they were chosen to study 
\1 Mentioning that we demonstrate for ELFO and CSAC, but our time-transfer framework would be applicable to any orbit type and clock type.
\end{outline}

\subsection{Lunar spaceborne GPS receiver modeling}
\begin{outline}
\1 STK stuff
    \2 Receiver antenna --> high-gain antenna -> modeled in STK 14 dBi.
    \2 path loss calculations -> C/N0 calculation, received power
    \2 steering antenna -> servo motor 
\1 MATLAB (Tara)
    \2 mention briefly again that modeling the residual pseudorange/Doppler calculations, based on GPS/lunar satellite ephemeris information
    \2 correlated error in lunar satellite ephemeris --> note difference from estimator, in EKF still consider it to be independent, given that noise is dominated by other tracking loop errors from low received C/N0
    \2 Currently, just modeling tracking loop error in Doppler measurements. Maybe can mention future work for velocity errors b/w GPS/lunar satellites
\end{outline}

\section{Experimental Results and Analysis}
\subsection{Implementation details}
\begin{outline}
\1 MATLAB to simulate plant model of GPS receiver and onboard clocks, and their associated errors. 
\1 values considered for lunar URE
\2 Earth-GPS URE values considered
\3 Simulation time duration is 2 months and sampling time is 60s. 
\end{outline}
\subsection{Validation metrics}
\begin{outline}
\1 Max ECOP 
\1 Max Timing errors observed --> across orbits 
\1 lunar URE depends on RMS timing error 
\end{outline}

\subsection{Results and Discussion}
\begin{outline}
\1 Max ECOP across different orbits 
\1 Timing errors: sensitivity across different ELFO orbits
\1 lunar URE metric
\end{outline}

\section{Conclusions and Future Work}

==> old_sections/simModeling.tex <==
\section{Modeling the Lunar Simulation Setup} \label{sec:simulation_modeling}

We design a high-fidelity lunar simulation environment using the Systems Tool Kit~(STK) software by the Analytical Graphics, Inc.~(AGI)~\cite{stk}. 
This simulation scenario is an extension of the validation setup designed for our earlier work~\cite{bhamidipati2021design}. 
We set the start time to be $9$ Nov $2025$ $00:00:00.000$ UTC and the experiment time duration to be $2$ months~(which equals $61$~days).
As described in Section~\ref{sec:intro}, we consider the LNSS satellite to be equipped with a low-SWaP onboard clock and a spaceborne Earth-GPS receiver.
Given an LNSS satellite orbit and clock, our simulation environment in STK models the transmission and reception of Earth-GPS signals to simulate the associated visibility and $\cno$ statistics.

%In particular, we model the following aspects: orbits of the Earth-GPS and LNSS satellites, transmit power and antenna gain patterns for the main lobe and side lobes of each Earth-GPS satellite, attenuation of Earth-GPS signals due to free-space path loss, occultation due to the Earth and the Moon, and spaceborne Earth-GPS receiver characteristics, such as antenna gain, tracking time. 

First, we design our simulated Earth-GPS constellation to be made up of $31$ operational satellites allocated in $6$ orbital planes as seen in Fig.~\ref{fig:EarthGPSconstellation}.
We utilize almanac data to propagate the position and velocity states of the Earth-GPS satellites for the entire experiment duration.
Our Earth-GPS constellation comprises $8$ satellites from Block IIR, $7$ from IIRM, $12$ from IIF and $4$ from Block III. 
We model the transmit antenna of Earth-GPS satellites by utilizing the publicly-available transmit power and antenna gain patterns of the L1~C/A signals, which are made available from the NASA GPS Antenna Characterization Experiment~(ACE)~\cite{donaldson2020characterization}. 
An illustration of the antenna gain pattern for a Block IIR Earth-GPS satellite is shown in Fig.~\ref{fig:BlockIIR}.
\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/GPSConstellation.jpg}
		\caption{Earth-GPS constellation with $31$ satellites}
		\label{fig:EarthGPSconstellation}
	\end{subfigure}	
	\hspace{2mm}
	\begin{subfigure}[b]{0.43\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/AntennaGainPatternIIR.jpg}
		\caption{Antenna gain pattern of a Block IIR satellite}
		\label{fig:BlockIIR}
	\end{subfigure}
	\caption{Our simulated setup; a)~Earth-GPS with $31$ satellites; b)~Antenna gain pattern for Block IIR with transmit power of $15~$dBW; Here, an off-boresight angle of $0^{\circ}$ represents the nadir direction~(facing Earth) of Earth-GPS satellites, while $90^{\circ}$ points towards the Earth-GPS satellite velocity/anti-velocity direction. Since the NASA GPS ACE~\cite{donaldson2020characterization} has no experimental data for off-boresight angles of less than $16^\circ$, we assign the antenna gain value for these angles to be a constant value which is equal to the average value obtained for the $16^\circ$ off-boresight angle across azimuth values between $0^\circ$ and $360^\circ$. This approximation has minimal effects on the simulation, since off-boresight angles of less than $16^{\circ}$ primarily make up the part of main lobe that is largely occluded by the Earth.} 
	\vspace{-4mm}
	\label{fig:earthGPS_modeling}
\end{figure}

To maximize the visibility of Earth-GPS signals at the LNSS satellite, we simulate a spaceborne Earth-GPS receiver with a steering antenna that is always pointed towards the Earth. 
We consider a high-gain antenna with $14$~\si{dBi} at $0^{\circ}$ off-boresight angle, and a $3~$dB beamwidth of $12.2^{\circ}$. 
As explained in~\cite{delepaut2020use}, this antenna pattern is representative of the current design of the Pretty CubeSat mission to be developed for GNSS reflectometry applications~\cite{fragner2020status}. 
Furthermore, in regard to the system noise temperature, we set a $30$~\si{dB} gain for the Low-Noise Amplifier~(LNA) with a noise figure of $2$~\si{dB} and an antenna noise temperature of $113$~\si{K}. 
We set the acquisition and tracking threshold for our simulated spaceborne Earth-GPS receiver as $15$~\si{dB-Hz}. 
%Fig.~\ref{fig:receivedCN0value} shows an example illustration of the received $\cno$, which is denoted by the orange dotted lines, from PRN $7$ of the Earth-GPS constellation in ELFO~\#1 while a threshold of $15~$dB-Hz is indicated by the black dashed line. 
We conservatively set the visibility condition such that an Earth-GPS satellite is considered to be visible when the received $\cno$ value is greater than $15$~\si{dB-Hz} for a continuous time duration of at least $40$~\si{s}.

% Didn't change this paragraph from ION GNSS+
To simulate the received Earth-GPS measurements utilized in the measurement update step described earlier in Section~\ref{sec:measurementupdate}, we first obtain the true range and true range rate between the Earth-GPS and LNSS satellites from STK and incorporate the simulated true clock bias and clock drift, as explained previously in Section~\ref{sec:modelingLNSSorbitclock}. 
To generate pseudorange residuals, we then subtract the true range measurements with that of the expected ones computed using the Earth-GPS and LNSS satellite ephemeris from STK, while introducing stochastic errors according to the measurement error model described in Eqs.~\eqref{eq:pseudorangecov}. 
For the LNSS satellite ephemeris error, we sample this component of the error residual only once per time step and incorporate the same measurement bias across all the simulated Earth-GPS pseudorange residuals. 
As a result, the simulated measurement residual vector~$z_t$ will have correlated errors; however, while formulating the measurement covariance matrix $\meascov\tidx{t}$ of our timing filter, we model the measurements as having uncorrelated errors. 
For the pseudorange rate residual measurements, we subtract the true range rate measurements with that of the expected ones, and thereafter induce stochastic errors based on only the simulated uncertainties from the PLL tracking loops.

A more detailed explanation regarding the modeling aspects of the transmit and the receiver antenna has been discussed in our earlier work~\cite{bhamidipati2021design}. 

To design an LNSS with time-transfer from Earth-GPS, we analyze the trade-off between different design considerations related to the onboard clock and the orbit type. 
An overview of the different case studies investigated in this work are explained below. 

\subsection{Formulating Case Studies by Varying Orbit and Clock of the LNSS Satellite} \label{sec:modelingLNSSorbitclock}

We create realistic simulations for an LNSS satellite in different lunar orbits by utilizing the High Precision Orbit Propagator~(HPOP) setting in the STK software~\cite{stk}. 
The HPOP builds upon precise force models of Earth, the Sun and the Moon for generating and propagating accurate orbit solutions of the LNSS satellite position and velocity~\cite{chao2000independent}. 

As mentioned in Section~\ref{sec:intro}, many prior studies~\cite{delepaut2020use,schonfeldt2020across} have investigated various types of lunar orbits, primarily based on their stability and the duration for which their stability can be ensured. 
Our choice of orbit types for this work include ELFO, NRHO, LLO and PCO.
Among them, we model the three orbit types, namely ELFO, LLO and PCO, in STK using classical orbit mechanics~\cite{montenbruck2012satellite}, which states that any orbit requires six elements (i.e., Keplarian parameters) to propagate the position and the motion of the LNSS satellite fully. 
Fig.~\ref{fig:LNSSsatelliteThreeOrbitTypes} shows an illustration of the three orbit types in the Moon-inertial frame.
Specifically, we refer to prior literature~\cite{ely2006constellations,delepaut2019system,whitley2016options} for the associated Keplarian parameters, which include the semi-major axis, eccentricity, inclination, argument of perigee, Right Ascension of the Ascending Node~(RAAN), and mean anomaly, and are listed in Table~\ref{table:LNSSsatorbits}. 

\begin{figure}[H]
\centering
\includegraphics[width=0.45\textwidth]{figures/MoonInertial_OthersModified.png}
\caption{Illustration of the three~(ELFO, LLO and PCO) among the four orbit types considered in our case study analysis.
All these orbits are visualized in the Moon-inertial frame, where ELFO indicated in orange is at an altitude of $9750.5$~\si{km}, LLO represented in magenta is at $100$~\si{km}, and PCO represented in blue is at $3000$~\si{km}. }
\label{fig:LNSSsatelliteThreeOrbitTypes}
\vspace{-3mm}
\end{figure}
\vspace{-4mm}
\begin{table}[H]
\centering
\caption{Keplarian parameters associated with the three~(ELFO, LLO and PCO) among the four case studies of orbit types considered.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Orbit Type \\ \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Altitude \\ (\si{km})\end{tabular}} & \textbf{Eccentricity} & \textbf{\begin{tabular}[c]{@{}c@{}}Inclination\\ ($^{\circ}$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Argument of\\ Perigee ($^{\circ}$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RAAN \\ ($^{\circ}$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean Anomaly\\ ($^{\circ}$)\end{tabular}} \\ \hline
\textbf{ELFO} & 9750.5 & 0.7 & 63.5 & 90 & 0 & 0 \\ \hline
\textbf{LLO} & 100 & 0 & 28.5 & 0 & 0 & 0 \\ \hline
\textbf{PCO} & 3000 & 0 & 75 & 0 & 90 & 0 \\ \hline
\end{tabular}
\label{table:LNSSsatorbits}
\end{table}

\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.92\textwidth]{figures/MoonInertial_NRHO.jpg}
		\caption{NRHO orbit type in Moon-inertial frame}
		\label{fig:LNSSsatelliteNRHOMoonIntertial}
	\end{subfigure}	
	\hspace{2mm}
	\begin{subfigure}[b]{0.43\textwidth}
		\includegraphics[width=0.98\textwidth]{figures/MoonCenteredRotatingFrame_NRHO.jpg}
		\caption{NRHO orbit type in Moon-centered Earth-Moon rotating frame}
		\label{fig:LNSSsatelliteNRHOEarthMoonRotating}
	\end{subfigure}
	\caption{The NRHO~(L2, radius of perigee=$4500$~\si{km}, South family) visualized in (a)~Moon-Inertial frame; and (b)~Moon-Centered Earth-Moon rotating frame.
	The x-axis of the Earth-Moon rotating frame is along the instantaneous Earth-Moon position vector, the z-axis is along the instantaneous angular momentum vector of the Moon’s orbit around the Earth, and the y-axis completes the orthogonal system.} 
	\label{fig:LNSSsatelliteNRHO}
\end{figure}
In contrast, for modeling the fourth orbit type in our case study, namely L2 South NRHO, we specify the initial conditions of position~$[r_x, r_y, r_z]$, and velocity~$[v_x, v_y, v_z]$ in a Moon-centered Earth-Moon rotating coordinate frame. 
Defining the initial conditions in an Earth-Moon rotating frame is particularly useful when discussing halo orbits in the Earth-Moon system. 
The x-axis of this frame is defined to be along the instantaneous Earth-Moon position vector, the z-axis is along the instantaneous angular momentum vector of the Moon’s orbit around the Earth, and the y-axis completes the orthogonal system.
Specifically, we refer to prior literature~\cite{williams2017targeting} that solves for an NRHO in the ephemeris model~(L2, radius of perigee to be $4500$~\si{km}, South family) using a forward/backward shooting process to provide the following initial state vector at an initial time epoch of $8$ Nov $2025$ $23:22:07.10353~$TDB:~$r_x=-125.952$~\si{km}, $r_y=120.961$~\si{km}, $r_z=4357.681~$km, $v_x=-0.042$~\si{km/s}, $v_y=1.468$~\si{km/s} and $v_z=-0.003$~\si{km/s}.%$r_x=-125.9522004870315$~\si{km}, $r_y=120.9609406690672$~\si{km}, $r_z=4357.680596646485~$km, $v_x=-0.04229621580376978$~\si{km/s}, $v_y=1.468560523456590$~\si{km/s} and $v_z=-0.003.538768970252955$~\si{km/s}.
An illustration of the designed NRHO orbit, both in the Moon-inertial frame~(similar frame as that in Fig.~\ref{fig:LNSSsatelliteThreeOrbitTypes}) and in the Moon-Centered Earth-Moon rotating frame are shown in Figs.~\ref{fig:LNSSsatelliteNRHOMoonIntertial} and~\ref{fig:LNSSsatelliteNRHOEarthMoonRotating}, respectively.

Given the SmallSat platform for the LNSS, we choose various case studies for clock types while keeping in mind that the limited payload capacity restricts the SWaP of the onboard clock.
We refer to prior literature~\cite{schmittberger2020review} to choose five case studies of onboard clocks, which for convenience have arranged in the increasing order of their SWaP characteristics in Table~\ref{table:LNSSsatclocks}. 
The chosen clock types include Microchip Chip Scale Atomic Clock~(CSAC), Microchip Micro Atomic Clock~(MAC), Stanford Research Systems~(SRS) PRS-10, Excelitas Rubidium Atomic Frequency Standard~(RAFS) and NASA's Deep Space Atomic Clock~(DSAC)~\cite{ely2018using,ely2014advancing}.
For the onboard clock, we model the true clock model as having a constant drift in the clock bias, with the propagation model defined in Eq.~\eqref{eq:pred_state}.
In particular, we model the constant drift to be equal to the TDEV, in order to observe the average drift consistent with the true clock error model. 
However, for our timing filter, we utilize the power spectral density coefficients listed in Table~\ref{table:LNSSsatclocks} to model the covariance matrix~$Q$ defined in Eq.~\eqref{eq:def_propcov}.

\begin{table}[H]
\centering
\caption{SWaP characteristics, time deviation and power spectral density coefficients of the five clock types considered in our case study analysis. 
SWaP and TDEV values are taken from~\cite{schmittberger2020review} while power spectral density coefficients were computed from their respective Allan deviation plots.}
\begin{tabular}{|c|c|c|c|c|ccc|}
\hline
\multirow{3}{*}{\textbf{Clock type}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Size\\ (\si{cm^3})\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ (\si{kg})\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Power\\ (\si{W})\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Time Deviation\\ (TDEV)~(\si{\mu s})\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Power Spectral Density Coefficients}} \\ \cline{6-8} 
 &  &  &  &  & \multicolumn{1}{c|}{\multirow{2}{*}{$h_{0}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$h_{-1}$}} & \multirow{2}{*}{$h_{-2}$} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{2}{*}{\textbf{Microchip CSAC}} & \multirow{2}{*}{17} & \multirow{2}{*}{0.035} & \multirow{2}{*}{0.1} & \multirow{2}{*}{1.5$\times10^{-6}$} & \multicolumn{1}{c|}{\multirow{2}{*}{1.3$\times 10^{-20}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{1.0$\times10^{-24}$}} & \multirow{2}{*}{3.7$\times10^{-29}$} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{2}{*}{\textbf{Microchip MAC}} & \multirow{2}{*}{50} & \multirow{2}{*}{0.084} & \multirow{2}{*}{5} & \multirow{2}{*}{1.7$\times 10^{-7}$} & \multicolumn{1}{c|}{\multirow{2}{*}{4.7$\times 10^{-22}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{1.2$\times 10^{-25}$}} & \multirow{2}{*}{1.7$\times10^{-30}$} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{2}{*}{\textbf{SRS PRS 10}} & \multirow{2}{*}{155} & \multirow{2}{*}{0.6} & \multirow{2}{*}{14.4} & \multirow{2}{*}{7.0$\times 10^{-8}$} & \multicolumn{1}{c|}{\multirow{2}{*}{1.3$\times10^{-22}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{2.3$\times10^{-26}$}} & \multirow{2}{*}{3.3$\times10^{-31}$} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{2}{*}{\textbf{Excelitas RAFS}} & \multirow{2}{*}{1645} & \multirow{2}{*}{6.35} & \multirow{2}{*}{39} & \multirow{2}{*}{4.8$\times10^{-9}$} & \multicolumn{1}{c|}{\multirow{2}{*}{8.0$\times10^{-24}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{0}} & \multirow{2}{*}{0} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{2}{*}{\textbf{NASA DSAC}} & \multirow{2}{*}{17000} & \multirow{2}{*}{16} & \multirow{2}{*}{47} & \multirow{2}{*}{4.0$\times10^{-11}$} & \multicolumn{1}{c|}{\multirow{2}{*}{1.8$\times10^{-27}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{0}} & \multirow{2}{*}{0} \\
 &  &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}
\label{table:LNSSsatclocks}
\end{table}


% Maybe not needed
% In our simulation, we mitigate the terrestrial ionospheric and tropospheric effects in the Earth-GPS signals by considering an Earth mask.
% We execute this by disregarding Earth-GPS signals that pass by the Earth at altitudes less than or equal to a pre-specified value of Earth mask. 
% Since the troposphere stretches up to $10~$km and the ionosphere extends up to $965~$km above Earth's surface, we choose an Earth mask of $965~$km.
% Note that, instead of disregarding these signals, modeling atmosphere effects is another viable option, which is left as an extension for future work.
% While our current paper only considers the Earth-GPS, note that our proposed time-transfer can be extended to include other Earth-GNSS constellations as well.%These aspects will be considered as extensions for future work. 

% \begin{figure}[H]
% 	\centering
% 	\begin{subfigure}[b]{0.49\textwidth}
% 		\includegraphics[width=0.98\textwidth]{figures/GPSConstellation.jpg}
% 		\caption{Earth-GPS constellation with $31$ satellites}
% 		\label{fig:EarthGPSconstellation}
% 	\end{subfigure}	
% 	\hspace{2mm}
% 	\begin{subfigure}[b]{0.43\textwidth}
% 		\includegraphics[width=0.98\textwidth]{figures/AntennaGainPatternIIR.jpg}
% 		\caption{Antenna gain pattern for Block IIR}
% 		\label{fig:BlockIIR}
% 	\end{subfigure}
% 	\vfill
% 	\vspace{5mm}
% 	\begin{subfigure}[b]{0.43\textwidth}
% 		\includegraphics[width=0.98\textwidth]{figures/AntennaGainPatternIIRM.jpg}
% 		\caption{Antenna gain pattern for Block IIRM}
% 		\label{fig:BlockIIRM}
% 	\end{subfigure}
% 	\hspace{1mm}
% 	\begin{subfigure}[b]{0.43\textwidth}
% 		\includegraphics[width=0.98\textwidth]{figures/AntennaGainPatternIIF.jpg}
% 		\caption{Antenna gain pattern for Block IIF}
% 		\label{fig:BlockIIF}
% 	\end{subfigure}	
% 	\caption{Our simulated setup; a)~Earth-GPS with $31$ satellites; b)~Antenna gain pattern for Block IIR with transmit power of $15~$dBW; c)~Antenna gain pattern for IIRM with transmit power of $14.3~$dBW; and d)~Antenna gain pattern for IIF with transmit power of $14.3~$dBW; The Block III is assigned the same transmit power and gain pattern as that of Block IIF. Since the NASA GPS ACE~\cite{donaldson2020characterization} has no experimental data for off-boresight angles of less than $16^\circ$, we assign the antenna gain value for these angles to be a constant value which is equal to the average value obtained for the $16^\circ$ off-boresight angle across azimuth values between $0^\circ$ and $360^\circ$. This approximation has minimal effects on the simulation, since off-boresight angles of less than $16^{\circ}$ primarily make up the part of main lobe that is largely occluded by the Earth.} 
% 	\label{fig:earthGPS_modeling}
% \end{figure}

% \subsection{Modeling the Earth-GPS Constellation} \label{sec:EarthGPSconstellation}
% We utilize the almanac obtained from the online AGI server to propagate the position and velocity states of the Earth-GPS satellites for the desired experiment duration. 
% Specifically, we consider the date of the almanac to be $25$ Oct $2020$ $17:04:00.000$ UTC with week reference as $07$ Apr $2019$.

% We consider our simulated Earth-GPS constellation to be made up of $31$ operational satellites allocated in $6$ orbital planes as seen in Fig.~\ref{fig:EarthGPSconstellation}.
% Our Earth-GPS constellation comprises $8$ satellites from Block IIR, $7$ from IIRM, $12$ from IIF and $4$ from Block III. 
% We utilize the transmit power and antenna gain patterns of the L1~C/A signals for Blocks IIR, IIRM and IIF from the NASA GPS Antenna Characterization Experiment (ACE)~\cite{donaldson2020characterization} to model the transmit antenna onboard the Earth-GPS satellites in our simulation setup. 
% The illustrations of these antenna gain patterns along with the assigned transmit powers are provided in Figs.~\ref{fig:BlockIIR}-\ref{fig:BlockIIF}.
% For the sake of simulation simplicity, we assign the same antenna gain pattern for satellites in each block of Earth-GPS constellation, which is equivalent to the average experimental antenna gain pattern files made publicly-available by~\cite{donaldson2020characterization}. 
% Given that no data is publicly available for Block III satellites, we approximate the transmit antennae of Block III using the transmit power and average antenna gain pattern available in~\cite{donaldson2020characterization} for Block IIF. 

% The antenna gain pattern files in~\cite{donaldson2020characterization} only contain data for angles ranging between $16^{\circ}-90^{\circ}$ for off-boresight and $0^{\circ}-360^{\circ}$ for azimuth.
% Similar to the notation considered in~\cite{delepaut2020use}, an off-boresight angle of $0^{\circ}$ represents the nadir direction~(facing Earth) of the GPS satellites, while $90^{\circ}$ points towards the Earth-GPS satellite velocity/anti-velocity direction.
% Given that the NASA GPS ACE does not include data for off-boresight angles of less than $16^{\circ}$, we assign the antenna gain for any Earth-GPS satellite between $0^{\circ}-16^{\circ}$ with a constant value that equals the average value obtained for the $16^{\circ}$ off-boresight angle, across the azimuth values ranging between $0^{\circ}-360^{\circ}$. 
% This approximation has minimal effects on the simulation results, since off-boresight angles of less than $16^{\circ}$ primarily make up the part of main lobe that is largely occluded by the Earth.  

% \subsection{Modeling the LNSS Satellite: ELFO and CSAC} \label{sec:modelingLNSSorbitclock}

% We create realistic simulations for an LNSS satellite in different lunar orbits by utilizing the High Precision Orbit Propagator~(HPOP) setting in the STK software~\cite{stk}. 
% The HPOP builds upon precise force models of the Earth, the Sun and the Moon for generating and propagating accurate orbit solutions of the LNSS satellite position and velocity~\cite{chao2000independent}. 
% As mentioned earlier in Section~\ref{sec:intro}, ELFOs have been the subject of great interest for the LNSS as they are highly stable and require significantly fewer station keeping maneuvers as compared to other types of lunar orbits.
% We model ELFOs in STK using classical orbit mechanics, which states that any orbit requires six elements (i.e., Keplarian parameters) to propagate the position and motion of the satellite fully. 
% Specifically, we refer to prior literature~\cite{ely2006constellations,schonfeldt2020across} for the Keplarian parameters associated with each ELFO, which include the semi-major axis, eccentricity, inclination, argument of perigee, Right Ascension of the Ascending Node~(RAAN), and mean anomaly, and are listed in Table~\ref{table:LNSSsatELFOs}. 
% \begin{figure}[H]
% 	\setlength{\belowcaptionskip}{-4pt}
% 	\centering
% 	\includegraphics[width=0.55\textwidth]{figures/ELFOs.png}
% 	\caption{Illustration of three ELFOs considered for validating our proposed time-transfer technique, where ELFO~\#1 is at an altitude of $6541.4~$km, ELFO~\#2 is at $7500~$km and ELFO~\#3 is at $9750.5~$km.}
% 	\label{fig:ELFOs}
% \end{figure}

% Fig.~\ref{fig:ELFOs} shows an illustration of the three ELFOs in the Moon-inertial frame.
% Particularly, we choose these three ELFOs given their persistent coverage of the South pole, which is a key region of interest for future lunar missions due to the presence of water ice deposits~\cite{li2018direct}. 
%As the LNSS satellite moves along an ELFO, the number of visible Earth-GPS satellites vary. 
% We conduct our experiments for LNSS satellite in ELFO and with an onboard CSAC, but in general, our proposed time-transfer technique would apply to any orbit and clock type. 
% Indeed, given the SmallSat platform for the LNSS, the limited payload capacity restricts the SWaP of the onboard clock, which makes CSAC a potentially useful option for a low-SWaP clock type.
% For our work, we simulate the onboard clock in accordance with the Microchip CSAC~\cite{lutwak2011sa}, which has a time deviation (TDEV) of $1.5$~\si{\mu s} per day and a SWaP of $(17$~\si{cm^3}$\cdot 0.0035$~\si{kg}$\cdot 0.12$~\si{W}$)$~\cite{schmittberger2020review}.
% For the onboard CSAC, we model the true clock model as having a constant drift in the clock bias, with the propagation model defined in Eq.~\eqref{eq:pred_state}.
% In particular, we model the constant drift to be equal to the TDEV, in order to observe the average drift consistent with the Microchip CSAC clock error model. However, for our timing filter, we utilize the covariance matrix model $Q$ defined in Eq.~\eqref{eq:def_propcov}, which has been derived in previous works.


% \subsection{Modeling the LNSS Satellite: Spaceborne Earth-GPS Receiver} \label{sec:modelingSpaceborneEarthGPSreceiver} 
% We simulate a spaceborne Earth-GPS receiver onboard an LNSS satellite in two parts: a)~we model the Earth-GPS signal reception in STK software, up to the computation of $\cno$ values; b)~we analyze the visibility statistics and induce simulated errors in pseudoranges and pseudorange rates in MATLAB, where the rest of our proposed time-transfer has been implemented. 

% To maximize the visibility of Earth-GPS signals at the LNSS satellite, we design a steering receiver antenna.
% In particular, we model steering characteristics by using an STK sensor object, mounting it on the LNSS satellite, and constraining it to always points towards the center of the Earth. 
% We then attach an STK receiver object on the sensor object, thereby ensuring that the Earth-GPS receiver onboard the LNSS satellite is always pointed towards the Earth. 
% We considered a high-gain antenna with $14~$dBi at $0^{\circ}$ off-boresight angle, and a $3~$dB beamwidth of $12.2^{\circ}$. 
% An illustration of the associated antenna gain pattern is shown in Fig.~\ref{fig:EarthGPSreceiverAntennaGain}.
% As explained in~\cite{delepaut2020use}, this antenna pattern is representative of the current design of the Pretty CubeSat mission to be developed for GNSS reflectometry applications~\cite{fragner2020status}. 
% Furthermore, in regard to the system noise temperature, we set a $30~$dB gain for the Low-Noise Amplifier~(LNA) with a noise figure of $2~$dB and an antenna noise temperature of $113~$K. For simplicity, we do not consider implementation losses and cable losses in our simulation. 
% \begin{figure}[H]
% 	\setlength{\belowcaptionskip}{-4pt}
% 	\centering
% 	\includegraphics[width=0.32\textwidth]{figures/ReceiverAntenna.jpg}
% 	\caption{Our simulated spaceborne Earth-GPS receiver is equipped with a high-gain steering receiver antenna with $14~$dBi at $0^{\circ}$ off-boresight angle, and a $3~$dB beamwidth of $12.2^{\circ}$.}
% 	\label{fig:EarthGPSreceiverAntennaGain}
% \end{figure}

% Prior work~\cite{musumeci2016design} demonstrated that acquisition and tracking can be achieved for a low $\cno$ threshold of $10~$dB-Hz while other works~\cite{blunt2016ultra,delepaut2020use} utilized a threshold of $15~$dB-Hz.
% To ensure a conservative margin, we set the acquisition and tracking threshold for our simulated spaceborne Earth-GPS receiver as $15~$dB-Hz. 
% Fig.~\ref{fig:receivedCN0value} shows an example illustration of the received $\cno$, which is denoted by the orange dotted lines, from PRN $7$ of the Earth-GPS constellation in ELFO~\#1 while a threshold of $15~$dB-Hz is indicated by the black dashed line. 
% We conservatively set the minimum required time duration of consistent signal visibility for acquisition and tracking to be $40~$s, i.e., a Earth-GPS satellite is considered to be visible when the received $\cno$ value is greater than $15~$dB-Hz for a continuous time duration of at least $40~$s. 

% To simulate the received Earth-GPS measurements utilized in the measurement update step described earlier in Section~\ref{sec:measurementupdate}, we first obtain the true range and true range rate between the Earth-GPS and LNSS satellites from STK and incorporate the simulated true clock bias and clock drift, as explained previously in Section~\ref{sec:modelingLNSSorbitclock}. 
% To generate pseudorange residuals, we then subtract the true range measurements with that of the expected ones computed using the Earth-GPS and LNSS satellite ephemeris from STK, while introducing stochastic errors according to the measurement error model described in Eqs.~\eqref{eq:pseudorangecov}-\eqref{eq:DLLcovariance}. 
% For the LNSS satellite ephemeris error, we sample this component of the error residual only once per time step and incorporate the same measurement bias across all the simulated Earth-GPS pseudorange residuals. 
% As a result, the simulated measurement residual vector~$z_t$ will have correlated errors; however, while formulating the measurement covariance matrix $\meascov\tidx{t}$ of our timing filter, we model the measurements as having uncorrelated errors. 
% For the pseudorange rate residual measurements, we subtract the true range rate measurements with that of the expected ones, and thereafter induce stochastic errors based on only the simulated uncertainties from the PLL tracking loops. Modeling other sources of uncertainties in the pseudorange rate residual, including lunar velocity estimation errors, is left as an extension for our future work.  %\tara{update mentioning errors of velocity ephemeris not included in our current work}.
% For the sake of simulation simplicity, we do not consider light time delay effects, i.e., change in position and velocity of the Earth-GPS satellite between the transmit time and received time at the LNSS satellite. 
% Incorporating light time delay to further improve the simulation setup has been left as an extension for future work. 



==> outline_IONITM.tex <==
\section{Introduction}
\begin{outline}[enumerate]
\1 Second space race / Motivation to return moon
    \2 Artemis mission
    \2 International goal for sustainable human presence on moon
    \2 60 upcoming mission...
    \2 South pole is a key interest region? (optional)

\1 Need for PNT for these missions
    \2 Near-term mission goals, need PNT for these missions
    \2 Earth has GPS
    \2 Can we have a GPS-like system for Moon?
        \3 In fact, NASA has lunaNet constellation. Interest in smallsats-> cost effectiveness and rapid deployment. 
    
\1 Questions we need to answer on how satellite navigation is different on Moon and what are its challenges? 
    \2 So many different orbits, which to choose? 
        \3 Some lunar orbits have previously been studied from different perspectives (stability, visibility) include: LLO, PCO, NRHO, ELFO
        \3 All of these have been studied, but which one do we choose?
        \3 (maybe remove?) Stability of orbit for longer durations, since no full-fledged ground infrastructure on Moon, similar to that of Earth. 
    \2 What clock do we choose? Need to choose good clock... This is particularly important as it affects the quality of ranging signals
    transmitted by the lunar navigation satellite...
    % \2 Given limited payload/SWaP capability of small satellite configuration and limited financial investment as compared to GPS military asset, which onboard clock to choose? This is particularly important as it affects the quality of ranging signals transmitted by the lunar navigation satellite.... not like GPS whose onboard clock is almost worth 200,000\$ (check?) and which is monitored using Earth ground stations twice every day using even more expensive clocks (which are the size of a refrigerator). --> maybe remove shoebox and $200000$  
    \2 Given limited payload/SWaP capability of small satellite configuration and limited financial investment / ground monitoring stations as compared to GPS (terrestrial, military asset), also need to be mindful of the challenges unique to lunar case/environment: less payload capacity / smaller satellites, less cost, less infrastructure for ground stations --> 
    \2 Given these challenges, can we harness the Earth-GPS, which is a established system, to alleviate/address some of these challenges while designing LNSS (from clock perspective).  

\1 Leveraging Earth-GPS on the Moon. 
    \2 Is this possible since main-lobe is occluded by Earth and Moon? Will the GPS signals be strong enough to navigate with at lunar distances?
    \2 Yes, it is possible. Many studies like NASA Navigator, ESA study analyzed the visibility of GPS signals at lunar distances. 
    \2 NASA ACE experiment also characterized the side-lobe performance and transmit antenna gain patterns.
    \2 Even though leveraging Earth-GPS signals is possible, Earth-GPS signals are not available at all times, only intermittently available with varying number of available measurements. 
    
\1 We design an LNSS propose a time-transfer technique from Earth-GPS to LNSS satellites.
    \2 We deal with intermittent availability via using timing-based kalman filter framework. 
    \2 We analyze trade-off between different design considerations related to orbits and clocks?
        \3 Many different orbits from among what has been explored in literature (NRHO, ELFO, LLO and PCO) 
            \4 Varying visibility of GPS satellites %to leverage timing ability
            \4 Develop ECOP metric to analyze effect of visibility on timing stability
        \3 Many different clock types
            \4 Size
            \4 Weight
            \4 Power
            \4 Timing stability
            \4 Include plot of SWaP vs timing -- highlight the 3 clock types on plot
            \4 Based on these criteria, CSAC, SRS and DSAC have been explored in existing literature. Describe the clocks and their importance. 
    \2 Specifically, we develop a lunar URE metric to characterize the trade-off
        
\1 Key contributions
    \2 Time-transfer technique to harness Earth-GPS signals
    \2 Timing-based filter technique to account for the intermittently available Earth-GPS signals, and when none available, propagating the clock estimates forward in time
    \2 Formulate lunar URE metric based on RMS timing error from time-transfer technique. 
    \2 Investigate design case studies for clocks and orbits (NRHO, ELFO, LLO and PCO). 
    \2 Simulated experiments to compare different case studies in terms of max ECOP, timing errors and lunar URE. 
\end{outline}

\section{Proposed Algorithm - Tara}
\subsection{Time-transfer/Estimator}
\begin{outline}
\1 EKF -> estimator clock and estimator measurement models (time and measurement update)
\1 process noise and measurement covariance formulation (high-level, symbolic representation of error terms / URE terms)
\1 Tracking loop values used / citation
\end{outline}
\subsection{lunar URE}
\begin{outline}
\1 Error budget terms which are present and not compared to Earth
\1 RMS timing error is added to broadcast clock 
\1 lunar URE expression is sum of four terms
\end{outline}

\section{Case studies: Orbits and Clocks - Ramya}
Clock modeled using MATLAB and orbits using STK. 
\begin{outline}
\1 Clocks modeling / case studies: 
    \2 Explain limitation of payload -- why considering smaller clocks
    \2 High-end of spectrum of clocks, new research clock DSAC -- trying to reduce the size, up-and-coming for space applications -- maybe mentioning that it depends on final decision of LunaNet satellite size which is not yet fixed
    \2 table of SWaP and timing stability of each clock (or perhaps a plot similar to arXiv study.)
    \2 True clock model based on time deviation --> Remarks about true vs estimator point out differences
\1 Orbit modeling / case studies: 
    \2 Start time of simulation considered (since NRHO depends on it?) 
    \2 Orbit types and details of each orbit. Perhaps orbit characteristics and why they were chosen to study 
    \2 Keplarian orbit based modeling for LLO, PCO.
    \2 ELFO and (need to check if its actually frozen or not!)
    \2 Moon-centered Earth-Moon rotating system L2 south lagrange points. Designing new axes based on barycenter of Earth-Moon.
    \2 (Min-Max) Altitude and time period of the different orbits
\end{outline}


\section{GPS receiver/transmitter Modeling/ Simulation}
\subsection{High-level Assumptions}
\begin{outline}
\1 Simulate (via STK) the visibility and C/N0 of received GPS signals in lunar regime, while modeling the following (high-level):
    \2 Occlusion of Earth/Moon, antenna gain patterns, free space path loss, attitude / geometry
\1 Assumption: Directly model the pseudorange and Doppler residual. 
\1 Consider earth mask to remove Earth ionospheric and tropospheric effects
\1 Tracking times of 36 s considered.
\end{outline}
\subsection{Earth-GPS constellation}
\begin{outline}
\1 Antenna gain patterns from NASA ACE study. Block III modeling using same antenna patterns as block IIF. How <16 deg stuff are modeled to have the same constant value. Transmit powers from GPS antenna for L1 C/A -- also only using L1 C/A
\1 Almanac year of 2019/2020? Based on this almanac, 31 satellites -- not using PRN 14 because it is decommissioned (or STK doesn't have this info)?
\end{outline}
\subsection{Lunar spaceborne GPS receiver modeling}
\begin{outline}
\1 STK stuff
    \2 Receiver antenna --> high-gain antenna -> modeled in STK 14 dBi.
    \2 path loss calculations -> C/N0 calculation, received power
    \2 steering antenna -> servo motor 
\1 MATLAB 
    \2 mention briefly again that modeling the residual pseudorange/Doppler calculations, based on GPS/lunar satellite ephemeris information
    \2 correlated error in lunar satellite ephemeris --> note difference from estimator, in EKF still consider it to be independent, given that noise is dominated by other tracking loop errors from low received C/N0
    \2 Currently, just modeling tracking loop error in Doppler measurements. Maybe can mention future work for velocity errors b/w GPS/lunar satellites
\end{outline}

\section{Experimental Results and Analysis}
\subsection{Implementation details}
\begin{outline}
\1 MATLAB to simulate plant model of GPS receiver and onboard clocks, and their associated errors. 
\1 values considered for lunar URE
\2 Earth-GPS URE values considered
\3 Simulation time duration is 2 months and sampling time is 60s. 
\end{outline}
\subsection{Validation metrics}
\begin{outline}
\1 Max ECOP 
\1 Max Timing errors observed --> across orbits and clocks
\1 lunar URE depends on RMS timing error 
\end{outline}

\subsection{Results and Discussion}
\begin{outline}
\1 Max ECOP across different orbits 
\1 Timing errors: Across different orbits
\1 Timing errors: Across different clocks
\1 lunar URE metric
\end{outline}

\section{Conclusions and Future Work}

==> outline_new_IONITM.tex <==
\section{Outline}

\begin{outline}
\1 Abstract --> Ramya-done
\1 Introduction --> More or less follow the ITM abstract, outline-IONITM file and our ION GNSS+ paper. --> Tara
    \2 Additionally, add the motivation about constellation design requires geometry and UERE --> in this work we look at UERE and thus, we work on one satellite analysis.
\1 Proposed Algorithm --> Tara
    \2 Summary of KF estimator -- same as ION GNSS+ \tara{can cite our paper instead of repeating everything? not sure what balance to have for the proposed algorithm, since would be empty if we remove too much}
    \2 Adaptive condition: If uncertainty as well as availability 
    \2 Inferences about the sensitivity of different components considered in lunar UERE --> Motivation for why we want to vary the broadcast ephemeris error or analyze our performance across different broadcast ephemeris error values. And why we are only varying broadcast ephemeris and not the others. --> Need literature survey for writing this part. 
\1 Modeling and Simulation setup --> Ramya
    \2 Summarize Earth-GPS constellation, LNSS receiver and true clock modeling. -- same as ION GNSS+ 
    \2 Add details about different LNSS orbit types in STK.
\1 Experiment Results and Analysis --> Ramya
    \2 Implementation details -- same as ION GNSS+
    \2 Plot for Earth-GPS visibility (one figure for each orbit) and table with sat visibility >=1 and >=4 and ECOP (with and without adaptive )
    \2 Plot for timing errors --> two figures (bias and drift) for each orbit and table for RMS characteristics --> with and without adaptive nature 
    \2 Plot of lunar UERE across clocks --> for different sensitivity analysis of ephemeris --> comment on hybrid characteristics of the lunar constellation
\1 Conclusions

~\\

\1 FUTURE EXPERIMENTS/THINGS TO ADD (after Dec 1)
    \2 Satellite footprint
    \2 Power consumption for antenna/signal transmission
    \2 Comment upon temporal perturbations-based on relativistic effects? 
    \2 Additional of L1 and DRO orbits based on thesis
    \2 Additional changes based on conversation with Prof.Axelrad (regarding clock) and Keidai (ephemeris error modeling-> any useful references) and Tyler Reid about modeling --> ephemeris error fit..?
\1 TO-DISCUSS:
        \2 What do you think about adaptive condition--> change in codes should be straightforward.
        \2 What internal timeline we should aim for --> Monday? Tuesday give to someone for read; incorporate edits and submit by Wednesday.
\end{outline}
